Soft-Constrained Optimization of Latent Space in Variational Autoencoders

The usefulness of a variational autoencoder (VAE) depends on two properties of its latent space that are hard to obtain together: high encoding capacity in the individual latent variables, and a low-dimensional, disentangled organization of those variables. Weakening the Kullback-Leibler regularization raises capacity but degrades disentanglement, while strengthening it prunes latent variables away entirely. We formulate VAE training as a soft-constrained optimization problem that addresses both. First, we impose an entropy-based constraint (EC) on individual latent variables, showing that the entropy of a latent code upper-bounds the mutual information it carries about the generative factors of the data. Second, we propose a weight-filter method that exploits the slack of the soft constraint to prune low-entropy dimensions during downstream training. On dSprites, the EC raises the aggregate latent-variable activation score by 43-62% over a vanilla VAE, attains the highest FactorVAE score among the \b{eta} \b{eta}-VAE variants (0.891 vs 0.847), and lowers reconstruction error by up to 38%. On MNIST, the weight filter reduces the latent dimensionality supplied to a downstream classifier from ten to two while holding accuracy above 90%, converging in 37% fewer epochs than the same procedure without the EC. We also find that low-entropy discrete factors tend to merge into a single latent variable, whereas high-entropy continuous factors are distributed across several.

==> table_backup.tex <==
\begin{table*}[htbp]
\begin{threeparttable}
%%Datafolder:  NewWork_Dz_10_bs64_epochs_200_seed1
\caption{Vanilla VAE Experimental Results with dSprites Dataset}
\label{table:vanillaresults}
\begin{tabular}{lcccccccccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{KKT Multipliers} & \multicolumn{3}{l}{Latent Variable Entropy} & \multicolumn{3}{c}{Disentanglement Score}               & \multicolumn{1}{l}{} \\ \hline
Model                & $\beta$    & $\gamma$   & $\delta$   & Ave.               & Min.     & Max.              & $\beta$-VAE Metric & FactorVAE Metric & Corr. Metric      & Reconstruction Error \\ \hline
Vanilla VAE          & 1          & 0          & 0          & 5.1163          & 4.9495          & \textbf{5.4181} & \textbf{0.5733}    & \textbf{0.7454}  & 3.6074          & 31.2481              \\
VAE+EC             & 1          & 1          & 0          & \textbf{5.3573} & \textbf{5.0792} & 5.4167          & 0.5272             & 0.7118           & 3.9361          & \textbf{19.4627}     \\
VAE+EC+LB             & 1          & 1          & 1          & 5.2349          & 5.0038          & 5.3474          & 0.5393             & 0.7115           & \textbf{4.1103} & 32.4894              \\
\hline
\end{tabular}
% \begin{tablenotes}
% \item
% EC: The entropy constraint of latent variables is imposed. 
% \item
% LB: The lower-bound of the latent variable entropy is set.
% \end{tablenotes}
\end{threeparttable}
\end{table*}

\begin{table*}[htbp]
\begin{threeparttable}
\centering
%%Datafolder: NewWork_Dz_10_bs64_epochs_200_seed10
\caption{$\beta$-VAE ($\beta=4$) Experimental Results with dSprites Dataset}
\label{table:beta4results}
\begin{tabular}{lcccccccccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{KKT Multipliers} & \multicolumn{3}{l}{Latent Variable Entropy}   & \multicolumn{3}{c}{Disentanglement Score}               & \multicolumn{1}{l}{} \\ \hline
Model                & $\beta$    & $\gamma$   & $\delta$   & Ave.            & Min.            & Max.            & $\beta$-VAE Metric & FactorVAE Metric & Corr. Metric      & Reconstruction Error \\ \hline
$\beta$-VAE          & 4          & 0          & 0          & 5.1432          & 4.9593          & 5.2201          & 0.5079             & 0.8468           & 4.0011          & 29.6556              \\
$\beta$-VAE+EC*            & 4          & 0.36       & 0          & 5.1743          & 5.0122          & 5.2302          & 0.4745             & 0.8682           & 3.6699          & 40.3712              \\
$\beta$-VAE+EC*+LB             & 4          & 0.36       & 1          & 5.1641          & 4.9239          & 5.2174          & \textbf{0.5118}    & 0.8449           & 3.8894          & \textbf{28.4817}     \\
$\beta$-VAE+EC             & 4          & 1          & 0          & 5.2386          & 5.0959          & 5.2796          & 0.4858             & \textbf{0.8907}  & \textbf{4.1268} & 35.2022              \\
$\beta$-VAE+EC+LB             & 4          & 1          & 1          & \textbf{5.2409} & \textbf{5.1566} & \textbf{5.2865} & 0.4172             & 0.8801           & 3.7112          & 46.1787   \\  
\hline
\end{tabular}
% \begin{tablenotes}
% \item
% EC: The entropy constraint of latent variables is imposed. 
% \item
% *: The KKT multiplier $\gamma$ is optimized.
% \item
% LB: The lower-bound of the latent variable entropy is set.
% \end{tablenotes}
\end{threeparttable}
\end{table*}
